Ion Alfv\'en velocity fluctuations and implications for the diffusion of streaming cosmic rays

The interstellar medium (ISM) of star-forming galaxies is magnetized and turbulent. Cosmic rays (CRs) propagate through it, and those with energies from $\sim\,\rm{GeV} - \rm{TeV}$ are likely subject to the streaming instability, whereby the wave damping processes balances excitation of resonant ionic Alfv\'en waves by the CRs, reaching an equilibrium in which the propagation speed of the CRs is very close to the local ion Alfv\'en velocity. The transport of streaming CRs is therefore sensitive to ionic Alfv\'en velocity fluctuations. In this paper we systematically study these fluctuations using a large ensemble of compressible MHD turbulence simulations. We show that for sub-Alfv\'enic turbulence, as applies for a strongly magnetized ISM, the ionic Alfv\'en velocity probability density function (PDF) is determined solely by the density fluctuations from shocked gas forming parallel to the magnetic field, and we develop analytical models for the ionic Alfv\'en velocity PDF up to second moments. For super-Alfv\'enic turbulence, magnetic and density fluctuations are correlated in complex ways, and these correlations as well as contributions from the magnetic fluctuations sets the ionic Alfv\'en velocity PDF. We discuss the implications of these findings for underlying "macroscopic" diffusion mechanisms in CRs undergoing the streaming instability, including modeling the macroscopic diffusion coefficient for the parallel transport in sub-Alfv\'enic plasmas. We also describe how, for highly-magnetized turbulent gas, the gas density PDF, and hence column density PDF, can be used to access information about ionic Alfv\'en velocity structure from observations of the magnetized ISM.

==> sim_table.tex <==
\def\arraystretch{1.35}
\LTcapwidth=\textwidth
\begin{ThreePartTable}
\footnotesize\setlength{\tabcolsep}{5pt}
\begin{TableNotes}
\item \textbf{\textit{Notes:}} All simulations listed are run with grid resolutions of $16^3$, $36^3$, $72^3$, $144^3$ and $288^3$. All statistics are spatially averaged over the entire domain, $\V = \V_{L}$, and are computed for 51 time realisations, across 5 correlation times of the Ornstein-Uhlenbeck forcing function. From the distributions in time, we report the values for the $16^{\rm th}$, $50^{\rm th}$, and $84^{\rm th}$ percentiles. This process minimises the possibility of using statistics that are undergoing temporally intermittent turbulent events \citep{Beattie2021b}. Column (1): the simulation ID, used throughout this study. Column (2): the turbulent Mach number, $\M \equiv \Exp{(\delta v / c_s)^2}^{1/2}_{\V_{L}}$. Column (3): the correlation scale of the turbulence, $\cor{v}$, in units of the driving scale, $\ell_0$, defined directly from the power spectra in \autoref{eq:correlation_scale}. Column (4): the Alfv\'en Mach number of the mean magnetic field, $\Mao \equiv \Exp{ (\delta v \sqrt{4\pi\rho_0} ) / B_0}$, with fluctuations coming from $\delta v$, since $\partial_{x_i}\mathbf{B}_0 = \partial_{t} \mathbf{B}_0 = 0$. Column (5): the mean magnetic field strength in units of $c_s \rho_0^{1/2}$. Column (6): the volume-averaged square of the turbulent magnetic field, proportional to the turbulent magnetic energy, in units of thermal energy. Column (7): the volume-averaged root-mean-squared of the magnetic coupling term $\dbBo$, in units of thermal energy. Column (8): the Alfv\'en Mach number of the turbulent magnetic field, \autoref{eq:turbMa}. Column (9): the Alfv\'en Mach number of the total magnetic field, \autoref{eq:totalMa}. 
\end{TableNotes}
\begin{longtable}{l r@{}l r@{}l c r@{}l r@{}l r@{}l r@{}l r@{}l}
\caption{Main simulation parameters and derived quantities used throughout this study.}\\
\hline
\hline
& \multicolumn{4}{c}{Turbulence} & \multicolumn{3}{c}{Large-scale $\mathbf{B}$-Field} & \multicolumn{6}{c}{Fluctuating $\mathbf{B}$-Field} & \multicolumn{2}{c}{Total $\mathbf{B}$-Field}\\
\hline\\
\multicolumn{1}{c}{Simulation ID} & \multicolumn{2}{c}{$\M$} & \multicolumn{2}{c}{$\frac{\ell_{\text{cor}, v}}{\ell_0}$} & \multicolumn{2}{c}{$\Mao$} & \multicolumn{1}{c}{$\frac{B_0}{c_s \rho_0^{1/2}}$} & \multicolumn{2}{c}{$\Exp{\frac{\delta B^2}{c_s^2 \rho_0}}_{\V}$} & \multicolumn{2}{c}{$\Exp{\left(\frac{\dB\cdot\Bo}{c_s^2 \rho_0}\right)^2 }^{1/2}_{\V}$} & \multicolumn{2}{c}{$\Maturb$} & \multicolumn{2}{c}{$\Matot$}\\
\multicolumn{1}{c}{(1)} & \multicolumn{2}{c}{(2)} & \multicolumn{2}{c}{(3)} & \multicolumn{2}{c}{(4)} & \multicolumn{1}{c}{(5)} & \multicolumn{2}{c}{(6)} & \multicolumn{2}{c}{(7)} & \multicolumn{2}{c}{(8)} & \multicolumn{2}{c}{(9)}\\[0.5em]
\hline
\texttt{M05MA001}&$0.567$ &$_{-0.07}^{+0.02}$&$1.48$ &$_{-0.07}^{+0.05}$&$0.0113$ &$_{-0.001}^{+0.0003}$&$177.0$&$0.000191$ &$_{-0.005}^{+0.004}$&$2.32$ &$_{-0.5}^{+0.4}$&$392.0$ &$_{-40.0}^{+20.0}$&$0.0113$ &$_{-0.001}^{+0.0003}$\\
\texttt{M05MA01}&$0.566$ &$_{-0.07}^{+0.02}$&$1.47$ &$_{-0.07}^{+0.05}$&$0.113$ &$_{-0.01}^{+0.004}$&$17.7$&$0.0181$ &$_{-0.04}^{+0.03}$&$2.23$ &$_{-0.4}^{+0.3}$&$35.6$ &$_{-2.0}^{+2.0}$&$0.113$ &$_{-0.01}^{+0.004}$\\
\texttt{M05MA05}&$0.534$ &$_{-0.04}^{+0.004}$&$1.44$ &$_{-0.07}^{+0.02}$&$0.534$ &$_{-0.04}^{+0.004}$&$3.54$&$0.233$ &$_{-0.08}^{+0.05}$&$1.16$ &$_{-0.1}^{+0.05}$&$7.28$ &$_{-0.2}^{+0.3}$&$0.544$ &$_{-0.05}^{+0.005}$\\
\texttt{M05MA1}&$0.469$ &$_{-0.05}^{+0.01}$&$0.953$ &$_{-0.005}^{+0.02}$&$0.938$ &$_{-0.1}^{+0.03}$&$1.77$&$1.2$ &$_{-0.3}^{+0.1}$&$1.0$ &$_{-0.07}^{+0.08}$&$2.75$ &$_{-0.2}^{+0.1}$&$0.974$ &$_{-0.08}^{+0.07}$\\
\texttt{M05MA2}&$0.462$ &$_{-0.03}^{+0.03}$&$0.783$ &$_{-0.03}^{+0.06}$&$1.85$ &$_{-0.1}^{+0.1}$&$0.886$&$3.17$ &$_{-0.3}^{+0.3}$&$0.871$ &$_{-0.07}^{+0.03}$&$1.67$ &$_{-0.08}^{+0.2}$&$1.59$ &$_{-0.09}^{+0.2}$\\
\texttt{M05MA4}&$0.473$ &$_{-0.03}^{+0.06}$&$0.838$ &$_{-0.03}^{+0.03}$&$3.79$ &$_{-0.2}^{+0.5}$&$0.443$&$3.12$ &$_{-0.2}^{+0.2}$&$0.415$ &$_{-0.009}^{+0.02}$&$1.98$ &$_{-0.2}^{+0.2}$&$2.1$ &$_{-0.2}^{+0.4}$\\
\texttt{M05MA6}&$0.483$ &$_{-0.03}^{+0.06}$&$0.904$ &$_{-0.03}^{+0.03}$&$5.8$ &$_{-0.4}^{+0.8}$&$0.295$&$2.74$ &$_{-0.1}^{+0.09}$&$0.256$ &$_{-0.006}^{+0.01}$&$2.32$ &$_{-0.1}^{+0.4}$&$2.51$ &$_{-0.2}^{+0.5}$\\
\texttt{M05MA8}&$0.502$ &$_{-0.02}^{+0.06}$&$0.907$ &$_{-0.02}^{+0.05}$&$8.03$ &$_{-0.3}^{+1.0}$&$0.222$&$2.47$ &$_{-0.2}^{+0.1}$&$0.192$ &$_{-0.01}^{+0.009}$&$2.76$ &$_{-0.1}^{+0.3}$&$2.99$ &$_{-0.2}^{+0.3}$\\
\texttt{M05MA10}&$0.514$ &$_{-0.03}^{+0.06}$&$0.934$ &$_{-0.03}^{+0.02}$&$10.3$ &$_{-0.5}^{+1.0}$&$0.177$&$2.24$ &$_{-0.07}^{+0.1}$&$0.145$ &$_{-0.006}^{+0.01}$&$3.05$ &$_{-0.2}^{+0.4}$&$3.18$ &$_{-0.1}^{+0.4}$\\
\texttt{M05MA100}&$0.637$ &$_{-0.05}^{+0.09}$&$0.889$ &$_{-0.03}^{+0.04}$&$127.0$ &$_{-10.0}^{+20.0}$&$0.0177$&$0.721$ &$_{-0.3}^{+0.1}$&$0.00852$ &$_{-0.001}^{+0.0008}$&$7.9$ &$_{-1.0}^{+3.0}$&$7.92$ &$_{-1.0}^{+3.0}$\\
\texttt{M05MA1000}&$0.672$ &$_{-0.05}^{+0.07}$&$0.835$ &$_{-0.04}^{+0.03}$&$1340.0$ &$_{-100.0}^{+100.0}$&$0.00177$&$0.36$ &$_{-0.3}^{+0.2}$&$0.000613$ &$_{-0.0002}^{+0.0001}$&$11.8$ &$_{-3.0}^{+8.0}$&$11.8$ &$_{-3.0}^{+8.0}$\\
\texttt{M2MA001}&$1.9$ &$_{-0.06}^{+0.04}$&$1.34$ &$_{-0.09}^{+0.02}$&$0.0095$ &$_{-0.0003}^{+0.0002}$&$709.0$&$0.000879$ &$_{-0.003}^{+0.02}$&$18.7$ &$_{-2.0}^{+9.0}$&$498.0$ &$_{-30.0}^{+20.0}$&$0.00943$ &$_{-0.0003}^{+0.0002}$\\
\texttt{M2MA01}&$1.85$ &$_{-0.02}^{+0.06}$&$1.37$ &$_{-0.1}^{+0.03}$&$0.0926$ &$_{-0.001}^{+0.003}$&$70.9$&$0.0989$ &$_{-0.03}^{+0.1}$&$18.4$ &$_{-1.0}^{+4.0}$&$41.1$ &$_{-3.0}^{+2.0}$&$0.0917$ &$_{-0.001}^{+0.003}$\\
\texttt{M2MA05}&$2.24$ &$_{-0.09}^{+0.07}$&$1.26$ &$_{-0.06}^{+0.08}$&$0.561$ &$_{-0.02}^{+0.02}$&$14.2$&$6.81$ &$_{-0.3}^{+0.3}$&$20.6$ &$_{-2.0}^{+3.0}$&$5.28$ &$_{-0.3}^{+0.3}$&$0.575$ &$_{-0.03}^{+0.01}$\\
\texttt{M2MA1}&$1.98$ &$_{-0.09}^{+0.1}$&$0.845$ &$_{-0.02}^{+0.02}$&$0.989$ &$_{-0.05}^{+0.05}$&$7.09$&$25.3$ &$_{-1.0}^{+0.3}$&$16.3$ &$_{-1.0}^{+0.7}$&$2.47$ &$_{-0.2}^{+0.2}$&$1.01$ &$_{-0.06}^{+0.05}$\\
\texttt{M2MA2}&$1.95$ &$_{-0.2}^{+0.2}$&$0.815$ &$_{-0.04}^{+0.04}$&$1.95$ &$_{-0.2}^{+0.2}$&$3.54$&$40.6$ &$_{-0.9}^{+0.6}$&$12.3$ &$_{-1.0}^{+0.7}$&$1.73$ &$_{-0.07}^{+0.4}$&$1.54$ &$_{-0.1}^{+0.1}$\\
\texttt{M2MA4}&$2.07$ &$_{-0.1}^{+0.2}$&$0.92$ &$_{-0.04}^{+0.02}$&$4.13$ &$_{-0.3}^{+0.5}$&$1.77$&$37.0$ &$_{-0.3}^{+0.3}$&$5.88$ &$_{-0.3}^{+0.4}$&$2.39$ &$_{-0.4}^{+0.1}$&$2.39$ &$_{-0.4}^{+0.3}$\\
\texttt{M2MA6}&$2.09$ &$_{-0.2}^{+0.2}$&$0.946$ &$_{-0.05}^{+0.02}$&$6.26$ &$_{-0.6}^{+0.6}$&$1.18$&$33.8$ &$_{-0.4}^{+0.5}$&$3.83$ &$_{-0.1}^{+0.1}$&$2.45$ &$_{-0.3}^{+0.5}$&$2.68$ &$_{-0.5}^{+0.6}$\\
\texttt{M2MA8}&$2.05$ &$_{-0.2}^{+0.09}$&$0.945$ &$_{-0.02}^{+0.04}$&$8.21$ &$_{-0.7}^{+0.4}$&$0.886$&$21.5$ &$_{-0.3}^{+0.3}$&$2.39$ &$_{-0.1}^{+0.1}$&$3.44$ &$_{-0.3}^{+0.2}$&$3.91$ &$_{-0.3}^{+0.2}$\\
\texttt{M2MA10}&$2.11$ &$_{-0.2}^{+0.1}$&$0.987$ &$_{-0.03}^{+0.03}$&$10.5$ &$_{-1.0}^{+0.7}$&$0.709$&$18.4$ &$_{-0.1}^{+0.3}$&$1.74$ &$_{-0.04}^{+0.1}$&$4.07$ &$_{-0.6}^{+0.3}$&$4.65$ &$_{-0.9}^{+0.4}$\\
\texttt{M2MA100}&$2.36$ &$_{-0.2}^{+0.1}$&$1.01$ &$_{-0.02}^{+0.03}$&$118.0$ &$_{-8.0}^{+6.0}$&$0.0709$&$3.3$ &$_{-0.5}^{+0.08}$&$0.0729$ &$_{-0.006}^{+0.003}$&$16.1$ &$_{-2.0}^{+3.0}$&$17.0$ &$_{-3.0}^{+4.0}$\\
\texttt{M2MA1000}&$2.37$ &$_{-0.1}^{+0.08}$&$0.999$ &$_{-0.05}^{+0.01}$&$1180.0$ &$_{-70.0}^{+40.0}$&$0.00709$&$0.276$ &$_{-0.3}^{+0.3}$&$0.00214$ &$_{-0.0007}^{+0.0005}$&$61.9$ &$_{-20.0}^{+40.0}$&$62.8$ &$_{-20.0}^{+40.0}$\\
\texttt{M4MA01}&$4.03$ &$_{-0.5}^{+0.06}$&$1.39$ &$_{-0.09}^{+0.05}$&$0.101$ &$_{-0.01}^{+0.002}$&$142.0$&$0.838$ &$_{-0.4}^{+0.2}$&$106.0$ &$_{-20.0}^{+9.0}$&$36.5$ &$_{-3.0}^{+3.0}$&$0.1$ &$_{-0.01}^{+0.002}$\\
\texttt{M4MA05}&$4.08$ &$_{-0.1}^{+0.04}$&$1.27$ &$_{-0.1}^{+0.04}$&$0.51$ &$_{-0.01}^{+0.005}$&$28.4$&$24.4$ &$_{-0.6}^{+0.4}$&$74.1$ &$_{-7.0}^{+7.0}$&$4.94$ &$_{-0.4}^{+0.3}$&$0.513$ &$_{-0.01}^{+0.007}$\\
\texttt{M4MA1}&$4.12$ &$_{-0.4}^{+0.5}$&$0.832$ &$_{-0.04}^{+0.04}$&$1.03$ &$_{-0.09}^{+0.1}$&$14.2$&$84.3$ &$_{-2.0}^{+2.0}$&$61.9$ &$_{-10.0}^{+7.0}$&$2.49$ &$_{-0.1}^{+0.3}$&$1.02$ &$_{-0.1}^{+0.05}$\\
\texttt{M4MA2}&$4.02$ &$_{-0.3}^{+0.2}$&$0.846$ &$_{-0.02}^{+0.04}$&$2.01$ &$_{-0.1}^{+0.08}$&$7.09$&$125.0$ &$_{-1.0}^{+1.0}$&$43.4$ &$_{-6.0}^{+2.0}$&$1.93$ &$_{-0.1}^{+0.2}$&$1.49$ &$_{-0.1}^{+0.2}$\\
\texttt{M4MA4}&$4.03$ &$_{-0.4}^{+0.2}$&$0.916$ &$_{-0.03}^{+0.02}$&$4.03$ &$_{-0.4}^{+0.2}$&$3.54$&$109.0$ &$_{-0.5}^{+0.2}$&$20.3$ &$_{-0.5}^{+2.0}$&$2.38$ &$_{-0.3}^{+0.1}$&$2.41$ &$_{-0.3}^{+0.1}$\\
\texttt{M4MA6}&$3.97$ &$_{-0.4}^{+0.2}$&$0.959$ &$_{-0.02}^{+0.02}$&$5.96$ &$_{-0.6}^{+0.3}$&$2.36$&$76.3$ &$_{-0.6}^{+0.3}$&$11.7$ &$_{-0.4}^{+0.7}$&$2.94$ &$_{-0.3}^{+0.4}$&$3.29$ &$_{-0.2}^{+0.4}$\\
\texttt{M4MA8}&$4.05$ &$_{-0.5}^{+0.08}$&$0.979$ &$_{-0.03}^{+0.02}$&$8.1$ &$_{-1.0}^{+0.2}$&$1.77$&$68.5$ &$_{-0.4}^{+0.6}$&$8.38$ &$_{-0.3}^{+0.3}$&$3.41$ &$_{-0.6}^{+0.3}$&$4.15$ &$_{-1.0}^{+0.4}$\\
\texttt{M4MA10}&$3.91$ &$_{-0.2}^{+0.2}$&$0.994$ &$_{-0.01}^{+0.03}$&$9.78$ &$_{-0.6}^{+0.5}$&$1.42$&$59.7$ &$_{-0.2}^{+0.2}$&$6.27$ &$_{-0.3}^{+0.2}$&$3.69$ &$_{-0.1}^{+0.3}$&$4.23$ &$_{-0.3}^{+0.9}$\\
\texttt{M4MA100}&$4.21$ &$_{-0.08}^{+0.2}$&$1.02$ &$_{-0.02}^{+0.03}$&$105.0$ &$_{-2.0}^{+5.0}$&$0.142$&$6.29$ &$_{-0.4}^{+0.4}$&$0.203$ &$_{-0.01}^{+0.01}$&$21.0$ &$_{-2.0}^{+3.0}$&$24.2$ &$_{-2.0}^{+5.0}$\\
\texttt{M4MA1000}&$4.31$ &$_{-0.2}^{+0.1}$&$1.05$ &$_{-0.01}^{+0.02}$&$1080.0$ &$_{-50.0}^{+30.0}$&$0.0142$&$0.391$ &$_{-0.3}^{+0.4}$&$0.00519$ &$_{-0.001}^{+0.001}$&$115.0$ &$_{-40.0}^{+20.0}$&$128.0$ &$_{-50.0}^{+30.0}$\\
\texttt{M6MA01}&$6.96$ &$_{-0.8}^{+0.5}$&$1.35$ &$_{-0.04}^{+0.05}$&$0.116$ &$_{-0.01}^{+0.008}$&$213.0$&$3.86$ &$_{-0.7}^{+0.3}$&$325.0$ &$_{-60.0}^{+20.0}$&$29.0$ &$_{-3.0}^{+4.0}$&$0.115$ &$_{-0.01}^{+0.008}$\\
\texttt{M6MA05}&$6.44$ &$_{-0.1}^{+0.2}$&$1.21$ &$_{-0.04}^{+0.02}$&$0.536$ &$_{-0.01}^{+0.02}$&$42.5$&$58.0$ &$_{-0.7}^{+1.0}$&$169.0$ &$_{-10.0}^{+10.0}$&$5.02$ &$_{-0.3}^{+0.3}$&$0.535$ &$_{-0.01}^{+0.01}$\\
\texttt{M6MA1}&$6.01$ &$_{-0.8}^{+0.8}$&$0.844$ &$_{-0.02}^{+0.04}$&$1.0$ &$_{-0.1}^{+0.1}$&$21.3$&$157.0$ &$_{-4.0}^{+1.0}$&$121.0$ &$_{-20.0}^{+10.0}$&$2.73$ &$_{-0.2}^{+0.2}$&$0.937$ &$_{-0.2}^{+0.1}$\\
\texttt{M6MA2}&$5.81$ &$_{-0.3}^{+0.3}$&$0.844$ &$_{-0.03}^{+0.03}$&$1.94$ &$_{-0.09}^{+0.1}$&$10.6$&$217.0$ &$_{-0.5}^{+2.0}$&$83.7$ &$_{-5.0}^{+9.0}$&$2.1$ &$_{-0.1}^{+0.2}$&$1.58$ &$_{-0.09}^{+0.09}$\\
\texttt{M6MA4}&$6.23$ &$_{-0.4}^{+0.1}$&$0.94$ &$_{-0.01}^{+0.02}$&$4.15$ &$_{-0.3}^{+0.08}$&$5.32$&$202.0$ &$_{-2.0}^{+0.8}$&$42.8$ &$_{-5.0}^{+2.0}$&$2.55$ &$_{-0.2}^{+0.2}$&$2.53$ &$_{-0.2}^{+0.3}$\\
\texttt{M6MA6}&$5.96$ &$_{-0.6}^{+0.4}$&$0.946$ &$_{-0.01}^{+0.02}$&$5.96$ &$_{-0.6}^{+0.4}$&$3.54$&$168.0$ &$_{-1.0}^{+1.0}$&$25.8$ &$_{-2.0}^{+3.0}$&$2.82$ &$_{-0.2}^{+0.3}$&$3.04$ &$_{-0.2}^{+0.3}$\\
\texttt{M6MA8}&$5.96$ &$_{-0.5}^{+0.2}$&$0.979$ &$_{-0.01}^{+0.01}$&$7.95$ &$_{-0.6}^{+0.2}$&$2.66$&$139.0$ &$_{-0.9}^{+0.3}$&$17.4$ &$_{-0.6}^{+1.0}$&$3.39$ &$_{-0.4}^{+0.2}$&$3.73$ &$_{-0.4}^{+0.2}$\\
\texttt{M6MA10}&$5.99$ &$_{-0.5}^{+0.2}$&$0.99$ &$_{-0.02}^{+0.02}$&$9.99$ &$_{-0.8}^{+0.4}$&$2.13$&$124.0$ &$_{-1.0}^{+0.5}$&$12.6$ &$_{-0.4}^{+1.0}$&$3.82$ &$_{-0.6}^{+0.8}$&$4.11$ &$_{-0.7}^{+1.0}$\\
\texttt{M8MA01}&$8.7$ &$_{-0.9}^{+0.09}$&$1.49$ &$_{-0.1}^{+0.02}$&$0.109$ &$_{-0.01}^{+0.001}$&$284.0$&$4.53$ &$_{-0.7}^{+0.4}$&$488.0$ &$_{-90.0}^{+40.0}$&$32.0$ &$_{-4.0}^{+4.0}$&$0.108$ &$_{-0.01}^{+0.001}$\\
\texttt{M8MA05}&$8.35$ &$_{-0.3}^{+0.2}$&$1.14$ &$_{-0.02}^{+0.02}$&$0.522$ &$_{-0.02}^{+0.01}$&$56.7$&$90.2$ &$_{-0.6}^{+1.0}$&$278.0$ &$_{-30.0}^{+20.0}$&$5.01$ &$_{-0.4}^{+0.3}$&$0.505$ &$_{-0.03}^{+0.01}$\\
\texttt{M8MA1}&$8.16$ &$_{-1.0}^{+0.6}$&$0.837$ &$_{-0.03}^{+0.04}$&$1.02$ &$_{-0.1}^{+0.08}$&$28.4$&$257.0$ &$_{-4.0}^{+2.0}$&$205.0$ &$_{-20.0}^{+10.0}$&$2.74$ &$_{-0.3}^{+0.3}$&$0.92$ &$_{-0.1}^{+0.07}$\\
\texttt{M8MA2}&$8.15$ &$_{-0.5}^{+0.4}$&$0.863$ &$_{-0.03}^{+0.03}$&$2.04$ &$_{-0.1}^{+0.1}$&$14.2$&$395.0$ &$_{-1.0}^{+1.0}$&$148.0$ &$_{-8.0}^{+7.0}$&$2.25$ &$_{-0.2}^{+0.2}$&$1.59$ &$_{-0.2}^{+0.1}$\\
\texttt{M8MA4}&$7.99$ &$_{-0.4}^{+0.3}$&$0.933$ &$_{-0.03}^{+0.01}$&$4.0$ &$_{-0.2}^{+0.1}$&$7.09$&$344.0$ &$_{-2.0}^{+0.8}$&$72.7$ &$_{-8.0}^{+4.0}$&$2.41$ &$_{-0.1}^{+0.2}$&$2.3$ &$_{-0.2}^{+0.2}$\\
\texttt{M8MA6}&$7.97$ &$_{-0.9}^{+0.4}$&$0.938$ &$_{-0.02}^{+0.02}$&$5.98$ &$_{-0.7}^{+0.3}$&$4.73$&$278.0$ &$_{-1.0}^{+2.0}$&$42.4$ &$_{-1.0}^{+7.0}$&$2.84$ &$_{-0.5}^{+0.2}$&$2.93$ &$_{-0.6}^{+0.3}$\\
\texttt{M8MA8}&$7.82$ &$_{-0.4}^{+0.4}$&$0.994$ &$_{-0.02}^{+0.01}$&$7.82$ &$_{-0.4}^{+0.4}$&$3.54$&$247.0$ &$_{-1.0}^{+0.8}$&$31.5$ &$_{-2.0}^{+2.0}$&$3.2$ &$_{-0.3}^{+0.2}$&$3.46$ &$_{-0.3}^{+0.5}$\\
\texttt{M8MA10}&$8.06$ &$_{-1.0}^{+0.2}$&$1.01$ &$_{-0.03}^{+0.02}$&$10.1$ &$_{-1.0}^{+0.3}$&$2.84$&$197.0$ &$_{-0.5}^{+1.0}$&$22.3$ &$_{-0.5}^{+1.0}$&$3.72$ &$_{-0.4}^{+0.6}$&$3.89$ &$_{-0.5}^{+0.6}$\\
\texttt{M10MA01}&$11.3$ &$_{-1.0}^{+0.3}$&$1.45$ &$_{-0.09}^{+0.07}$&$0.113$ &$_{-0.01}^{+0.003}$&$354.0$&$6.76$ &$_{-1.0}^{+1.0}$&$720.0$ &$_{-200.0}^{+100.0}$&$33.7$ &$_{-7.0}^{+8.0}$&$0.112$ &$_{-0.01}^{+0.003}$\\
\texttt{M10MA05}&$10.2$ &$_{-0.3}^{+0.3}$&$1.13$ &$_{-0.02}^{+0.02}$&$0.509$ &$_{-0.02}^{+0.01}$&$70.9$&$143.0$ &$_{-2.0}^{+2.0}$&$420.0$ &$_{-40.0}^{+20.0}$&$4.88$ &$_{-0.5}^{+0.6}$&$0.496$ &$_{-0.02}^{+0.02}$\\
\texttt{M10MA1}&$9.72$ &$_{-0.9}^{+0.9}$&$0.868$ &$_{-0.03}^{+0.03}$&$0.972$ &$_{-0.09}^{+0.09}$&$35.4$&$338.0$ &$_{-4.0}^{+3.0}$&$309.0$ &$_{-40.0}^{+20.0}$&$2.79$ &$_{-0.1}^{+0.4}$&$0.888$ &$_{-0.1}^{+0.06}$\\
\texttt{M10MA2}&$10.5$ &$_{-0.8}^{+0.3}$&$0.888$ &$_{-0.02}^{+0.02}$&$2.1$ &$_{-0.2}^{+0.07}$&$17.7$&$549.0$ &$_{-1.0}^{+0.9}$&$215.0$ &$_{-10.0}^{+9.0}$&$2.39$ &$_{-0.3}^{+0.1}$&$1.56$ &$_{-0.1}^{+0.2}$\\
\texttt{M10MA4}&$10.3$ &$_{-0.4}^{+0.4}$&$0.931$ &$_{-0.03}^{+0.03}$&$4.12$ &$_{-0.2}^{+0.2}$&$8.86$&$529.0$ &$_{-2.0}^{+2.0}$&$112.0$ &$_{-6.0}^{+8.0}$&$2.42$ &$_{-0.2}^{+0.4}$&$2.32$ &$_{-0.2}^{+0.4}$\\
\texttt{M10MA6}&$9.78$ &$_{-1.0}^{+0.3}$&$0.952$ &$_{-0.03}^{+0.02}$&$5.87$ &$_{-0.7}^{+0.2}$&$5.91$&$398.0$ &$_{-0.7}^{+2.0}$&$65.2$ &$_{-3.0}^{+7.0}$&$2.7$ &$_{-0.4}^{+0.3}$&$2.77$ &$_{-0.4}^{+0.3}$\\
\texttt{M10MA8}&$10.0$ &$_{-0.9}^{+0.4}$&$0.997$ &$_{-0.02}^{+0.02}$&$8.03$ &$_{-0.7}^{+0.3}$&$4.43$&$346.0$ &$_{-1.0}^{+1.0}$&$46.7$ &$_{-1.0}^{+4.0}$&$3.27$ &$_{-0.4}^{+0.4}$&$3.41$ &$_{-0.6}^{+0.4}$\\
\texttt{M10MA10}&$9.42$ &$_{-0.5}^{+0.2}$&$0.99$ &$_{-0.01}^{+0.01}$&$9.42$ &$_{-0.5}^{+0.2}$&$3.54$&$288.0$ &$_{-3.0}^{+2.0}$&$34.3$ &$_{-4.0}^{+3.0}$&$3.37$ &$_{-0.2}^{+0.3}$&$3.5$ &$_{-0.3}^{+0.5}$\\
\hline
\hline
\insertTableNotes
\label{tb:simtab}
\end{longtable}
\end{ThreePartTable}

